Introducing Dynamic Behavior in Amalgamated Knowledge Bases

The problem of integrating knowledge from multiple and heterogeneous sources is a fundamental issue in current information systems. In order to cope with this problem, the concept of mediator has been introduced as a software component providing intermediate services, linking data resources and application programs, and making transparent the heterogeneity of the underlying systems. In designing a mediator architecture, we believe that an important aspect is the definition of a formal framework by which one is able to model integration according to a declarative style. To this purpose, the use of a logical approach seems very promising. Another important aspect is the ability to model both static integration aspects, concerning query execution, and dynamic ones, concerning data updates and their propagation among the various data sources. Unfortunately, as far as we know, no formal proposals for logically modeling mediator architectures both from a static and dynamic point of view have already been developed. In this paper, we extend the framework for amalgamated knowledge bases, presented by Subrahmanian, to deal with dynamic aspects. The language we propose is based on the Active U-Datalog language, and extends it with annotated logic and amalgamation concepts. We model the sources of information and the mediator (also called supervisor) as Active U-Datalog deductive databases, thus modeling queries, transactions, and active rules, interpreted according to the PARK semantics. By using active rules, the system can efficiently perform update propagation among different databases. The result is a logical environment, integrating active and deductive rules, to perform queries and update propagation in an heterogeneous mediated framework.

==> Defs2.tex <==
\newcommand{\lgt}{$\cal T$}
\newcommand{\clc}{$\cal C$}
\newcommand{\clfi}{${\cal F}^i$}
\newcommand{\ag}{{\accent 18 a}}
\newcommand{\eg}{{\accent 18 e}}
\newcommand{\ig}{{\accent 18 \char 16}}
\newcommand{\og}{{\accent 18 o}}
\newcommand{\ug}{{\accent 18 u}}
\newcommand{\ea}{\'e}
\newcommand{\Iint}{i-in\-ter\-pre\-ta\-tion}
\newcommand{\rint}{r-in\-ter\-pre\-ta\-tion}
\newcommand{\rintp}{r-in\-ter\-pre\-ta\-tions}
\newcommand{\aint}{A-in\-ter\-pre\-ta\-tion}
\newcommand{\aintp}{A-in\-ter\-pre\-ta\-tions}
\newcommand{\bstr}{bi-struc\-tu\-re}
\newcommand{\iloc}{$I^{loc}$}
%\newcommand{\Ilocm}{I^{loc}}
\newcommand{\iaml}{$I^{aml}$}
%\newcommand{\Iamlm}{I^{aml}}
\newcommand{\ilocm}{I^{loc}}
\newcommand{\iamlm}{I^{aml}}
\newcommand{\lgtj}{${\cal T}_j$}
\newcommand{\lgtjm}{{\cal T}_j}
\newcommand{\lgtloc}{${\cal T}^{loc}$}
\newcommand{\lgtlocm}{{\cal T}^{loc}}
\newcommand{\lgl}{$\cal L$}
\newcommand{\lgtm}{{\cal T}}
\newcommand{\lglm}{\cal L}
\newcommand{\ulgl}{$U_{\cal L}$}
\newcommand{\blgl}{$B_{\cal L}$}
\newcommand{\ulglm}{U_{\cal L}}
\newcommand{\blglm}{B_{\cal L}}
\newcommand{\blgp}{$B_{\cal P}$}
\newcommand{\blgpm}{B_{\cal P}}
\newcommand{\clf}{$\cal F$}
\newcommand{\clfij}{${\cal F}^i_j$}
\newcommand{\clfijm}{{\cal F}^i_j}
\newcommand{\clfim}{{\cal F}^i}
\newcommand{\clfm}{\cal F}
\newcommand{\clcm}{\cal C}
\newcommand{\clp}{$\cal P$}
\newcommand{\clpm}{\cal P}
\newcommand{\clv}{$\cal V$}
\newcommand{\clvm}{\cal V}
\newcommand{\car}{$\{{\overleftarrow A},\{\alpha_1 D_1,\ldots,\alpha_k D_k\}\}$}
\newcommand{\ca}{$\{{\overleftarrow A},\{\alpha_1 D_1,\ldots,\alpha_k D_k\}\}$}
\newcommand{\caar}{$\langle\{{\overleftarrow A},\{\alpha_1 D_1,\ldots,\alpha_k D_k\}\},\{\psi,\{\mu_1,\ldots,\mu_k\}\}\rangle$}
\newcommand{\caa}{$\langle\{A,\{\alpha_1 D_1,\ldots,\alpha_k D_k\}\},\{\psi,\{\mu_1,\ldots,\mu_k\}\}\rangle$}
\newcommand{\carm}{\{{\overleftarrow A},\{\alpha_1 D_1,\ldots,\alpha_k D_k\}\}}
\newcommand{\cam}{\{{\overleftarrow A},\{\alpha_1 D_1,\ldots,\alpha_k D_k\}\}}
\newcommand{\caarm}{\langle\{{\overleftarrow A},\{\alpha_1 D_1,\ldots,\alpha_k D_k\}\},\{\psi,\{\mu_1,\ldots,\mu_k\}\}\rangle}
\newcommand{\caam}{\langle\{A,\{\alpha_1 D_1,\ldots,\alpha_k D_k\}\},\{\psi,\{\mu_1,\ldots,\mu_k\}\}\rangle}
\newcommand{\ac}{\hfill\break}
%\newcommand{\algorithm}{\obeylines\baselineskip=1cm\parindent=0.5cm\parskip0ex\small}
\newcommand{\ii}{\hspace*{0.3cm}}
\newcommand{\bfunc}{{\bf {function}\ }}
\newcommand{\breturn}{{\bf {return}\ }}
\newcommand{\band}{{\bf {and}\ }}
\newcommand{\bor}{{\bf {or}\ }}
\newcommand{\bnot}{{\bf {not}\ }}
\newcommand{\balgo}{{\bf {Algorithm}\ }}
\newcommand{\bbegin}{{\bf {begin}\ }}
\newcommand{\bend}{{\bf {end}\ }}
\newcommand{\blet}{{\bf {let}\ }}
\newcommand{\bif}{{\bf {if}\ }}
\newcommand{\bthen}{{\bf {then}\ }}
\newcommand{\belse}{{\bf {else}\ }}
\newcommand{\bendif}{{\bf {endif}\ }}
\newcommand{\bevery}{{\bf {every}\ }}
\newcommand{\binput}{{\bf {input}\ }}
\newcommand{\boutput}{{\bf {output}\ }}
\newcommand{\bmethod}{{\bf {method}\ }}
\newcommand{\real}{\rm I\kern-.2em R}
\newcommand{\nat}{{\rm I\kern-.2em N}}
\newcommand{\espace}{\rm I\kern-.2em E}
\newcommand{\Beginboxit}{\par\vbox\bgroup\hrule\hbox\bgroup\vrule \kern2.2pt \vbox\bgroup\kern2.2pt}
\newcommand{\Endboxit}{\kern2.2pt\egroup\kern2.2pt\vrule\egroup\hrule\egroup}

